Price Stability and Improved Buyer Utility with Presentation Design: A Theoretical Study of the Amazon Buy Box

Platforms design the form of presentation by which sellers are shown to the buyers. This design not only shapes the buyers' experience but also leads to different market equilibria or dynamics. One component in this design is through the platform's mediation of the search frictions experienced by the buyers for different sellers. We take a model of monopolistic competition and show that, on one hand, when all sellers have the same inspection costs, the market sees no stable price since the sellers always have incentives to undercut each other, and, on the other hand, the platform may stabilize the price by giving prominence to one seller chosen by a carefully designed mechanism. This calls to mind Amazon's Buy Box. We study natural mechanisms for choosing the prominent seller, characterize the range of equilibrium prices implementable by them, and find that in certain scenarios the buyers' surplus improves as the search friction increases.

==> camera_ready/conclusion.tex <==
We study the mechanism design problem for a two-sided online marketplace with search frictions on the buyer's side, exemplified by Amazon's business model and is canonical in digital economics. We propose a model that features multiple strategic sellers and utility maximizing buyers. Our model accounts for the buyer's optimal search behavior in the presence of inspection costs and sellers' strategic pricing behavior.
We characterize sellers' demand and revenue under these conditions, and analyze how the design of the Buy Box influences market outcomes, particularly focusing on price equilibria, social welfare, and consumer surplus.

The first part of our theoretical findings reveal that no symmetric equilibrium exists for markets with multiple sellers and that general equilibrium does not exist in the case of two sellers. This underscores the necessity of some mechanism to stabilize the market. 

Motivated by Amazon's approach, we study the design of Buy Box mechanisms. We first showed that the almost naive Lowest-Price-First mechanism does not sustain equilibrium. The inherent inspection cost boost Buy Box seller's demand, hence incentivizes sellers to constantly undercutting their prices to win the Buy Box. This finding aligns with the observed pricing chaos on Amazon, where frequent and significant price changes reflect the underlying instability in a market without an effective equilibrium mechanism.


To address this instability, we propose the Dictator-$t$ mechanism, which awards the Buy Box to sellers pricing at a pre-specified price point. This mechanism proves effective in being able to support the lowest equilibrium price among all anonymous mechanisms. We also examine the Threshold-$t$ mechanism, which selects sellers pricing below a specified threshold for the Buy Box. Although more flexible, this mechanism is less robust than the Dictator-$t$ mechanism, and does not achieve the same degree of low prices.

Furthermore, our analysis highlights the critical role of inspection costs in driving social welfare and consumer surplus. While in our model, higher inspection costs reduces social welfare, it lowers the incentive for buyers to conduct thorough searches, therefore, somewhat surprisingly, drives down equilibrium price and increases consumer surplus. This trade-off underscores the platform's strategic role in optimizing market outcomes by carefully calibrating the design of their display policy and user interface.

In conclusion, the Amazon Buy Box, when designed and implemented with consideration of inspection costs and appropriate mechanism, can significantly improve market efficiency and buyer utility. By establishing a model that incorporates both buyer and seller strategies, we provide a foundation for understanding how search frictions and platform design influence market outcomes. Future research can extend these insights by exploring dynamic pricing strategies and further empirical validation of the proposed mechanisms in diverse market settings. This study provides a critical framework for understanding the interplay between search frictions, platform design, and market outcomes in the digital economy.




==> camera_ready/intro.tex <==
\begin{quote}
    ``You may not realize it, but shopping on Amazon is more like playing the stock market than shopping at your local big box store... That’s because Amazon and the site’s third-party sellers are engaged in an algorithmically enabled pricing war.'' \\
    --- Kristen V. Brown (2016  \cite{brown2016amazon})
\end{quote}

Let's go shopping, online. When we have a demand for a certain consumer product, before actually making a purchase at a particular seller, we faces a non-negligible mental and temporal cost in screening the seller's offer. A consumer will have to consider reviews, product details, shipping terms, and after-sales guarantees. Often, this search-and-screen is non-exhaustive: that although there are tens or even thousands of sellers on the platform, mostly one sees only a small subset, and even frequently opting for the first link they encounter and makes a direct purchase.

Due to this information overflow, the platform's method of presenting sellers to consumers significantly impacts market outcomes. The graphic interface design—how much information is instantly presented and how conveniently more can be obtained—affects the consumer's shopping experience and purchase decisions. Moreover, the ranking algorithm, which may prioritize certain sellers, also substantially influences market outcomes.

Platforms like Amazon often seek to control market prices, typically aiming for lower prices to maximize consumer surplus and, consequently, their own popularity. This is because their long-term profit strategy relies on scaling up network effects, primarily by attracting more buyers.

The utility disjunction between the platform and the sellers creates a battle over market power over prices. The platform has influence via its interface design due to the information overflow in a thick seller market. To incentivize competitive prices, a natural approach might be to reward sellers offering lower prices with higher visibility. Various presentation choices could serve this goal. For instance, sellers with lower prices might be featured more prominently, reducing inspection costs for consumers. An extreme measure is to make one seller particularly prominent, such as displaying their information as the default choice and imposing inspection costs on all other sellers. Amazon’s \textbf{Buy Box} exemplifies this approach.


\subsection{Buy Box}

When a buyer reaches a landing page on \texttt{amazon.com} describing a particular product offered by possibly multiple sellers, say a particular book, the buyer is presented with a \textit{Buy Box} containing the price and the buttons the buyer should press if he is ready to purchase from the Buy Box seller (Figure \ref{fig:buy_box_demo-1} red region). Below the Buy Box, and typically not immediately visible without scrolling, an additional box (shown in the green region of Figure~\ref{fig:buy_box_demo-1}) offers purchase options from other sellers. Initially, this area displays only the lowest price available and provides limited details. Only when the buyer click open this additional box will the information and link of other sellers be displayed (Figure~\ref{fig:buy_box_demo-2}).


\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\linewidth]{figures/buy_box_demo-1.png} 
    \caption{Landing page}
    \label{fig:buy_box_demo-1}
    \includegraphics[width=0.45\linewidth]{figures/buy_box_demo-2.png} 
   \caption{The link to other buyers}
    \label{fig:buy_box_demo-2}
    \Description{This screenshots displays when a user searches a book on Amazon. For the landing page \ref{fig:buy_box_demo-1}, in red is the Buy Box section, which includes options such as 'Add to Cart' and 'Buy Now' buttons. To view alternative purchasing options from other sellers, users need to scroll down to the section marked in green.}
\end{figure}


By presenting the seller information in this way, Amazon is de facto reducing the inspection cost the buyer incurs to find the Buy Box seller, and hence increasing the chance of a sale to this seller. For other sellers of this same product, Amazon has, for all practical purposes, increased the inspection cost.

What change does the Buy Box cause to the market when compared with plainer interface, e.g. simply listing the link to all sellers without prioritizing one of them? To understand this, one must first consider how Amazon selects the Buy Box seller. According to Amazon's official guide \cite{Amazon2023BuyBox}, the platform considers various factors, including the seller's price, reputation, and shipping policies. However, the exact mechanism is proprietary.

The sellers and the platform are playing a game: Amazon designs a \textit{Buy Box mechanism} which specifies the procedure (possibly randomized) for mapping information about sellers and buyer to a Buy Box winner, and the sellers ``play'' the game. An empirical study~\cite{chen-algorithmic_pricing-2016} had documented the high-stakes, high-speed algorithmic pricing that is occurring on amazon.com. Third-party sellers on Amazon take advantage of pricing software to scrape other sellers' price information and help them update their prices incessantly –– so as to be favored by the Buy Box. Even Amazon offers free algorithmic pricing tool~\cite{amazon_automate_pricing} for sellers to `\textit{adjust your prices quickly and automatically against your competition to increase your chance of becoming the [Buy Box]}'.

% the line spacing here is weird. added this \newline to make it at least looks better
\paragraph{In this paper, we address two fundamental questions:}

\begin{enumerate}
    \item Is the Buy Box beneficial for the general two-sided platform e-commerce market?
    \item How can the platform design the Buy Box policy and adjust inspection difficulty to influence the market favorably?
\end{enumerate}

\subsection{Our Contributions}

\note{PENDING @HuFu}
% We model a market for a given product on Amazon as a monopolistic competition, where the buyer’s optimal strategy in presence of inspection cost is given by the \textit{Pandora’s Box algorithm}. We first analyze the market outcome without the Buy Box and show that it fails to admit any equilibrium price set by sellers. We then explore three Buy Box mechanisms. The first mechanism, despite widely applied and intuitive, admits no pure equilibrium. The second mechanism we demonstrate is the most effective among practical mechanisms, while the third, a generalized version of the first, is almost as effective in most cases.

% In a market with a limited number of sellers differentiated by service terms, reputation, and other features, we model this as monopolistic competition. The buyer's value for purchasing from a seller is a random variable independently drawn from a known distribution. Sellers set their prices, but buyers do not know the exact value until they inspect the sellers.

% The consumer's search problem is solved by Weitzman's elegant and simple Pandora’s Box algorithm, which we detail in Section~\ref{sec:pandoras_box}. This algorithm allows buyers to compute a reservation price that helps determine whether it is worthwhile to incur the screening cost.

% We begin by answering why a Buy Box mechanism is needed in the first place. We demonstrate that without the Buy Box, even minimal inspection costs lead to market failure. The subsequent problem is designing the Buy Box mechanism to foster market equilibrium and increase consumer surplus.

% We analyze the simplest mechanism --- awarding the Buy Box to the seller with the lowest price --- and show it has no pure symmetric equilibrium. This lack of equilibrium can partially explain the price fluctuations observed on Amazon. 

% We then focus on the \textit{Dictator} and \textit{Threshold} mechanisms. Both mechanisms are parameterized by a target price, with the Buy Box allocated to sellers who match (Dictator) or price below (Threshold) the target price. We prove that the Dictator mechanism always attains the lowest possible equilibrium prices, while the Threshold mechanism is nearly as effective. This allows us to understand the potential benefits of the Buy Box.

% Our analysis shows that increasing inspection costs may, counter intuitively, increase consumer surplus by lowering prices --- despite the externality of increased friction imposed on consumers. We characterized a sufficient condition for consumer surplus to be maximized at an intermediate level of inspection cost. We also characterized the platform's market power --- the range of prices it can control, and the market's achievable Pareto frontier via design of Buy Box mechanism.

% We see this work as a step toward understanding search frictions in platform interfaces and related mechanism design problems. Future work will address additional questions raised by our findings.

\subsection{Related Work}




==> camera_ready/newintro.tex <==
Platforms that enable transactions between buyers and providers have become major venues of the e-commerce. 
As a few salient examples, Amazon and eBay allow buyers to purchase from a vast body of sellers, and Airbnb connects travelers and hosts.  
An important activity on these websites is for one side of the market to search on the other side for a service or good.  
Search is sequential and time-consuming, and usually cannot be exhaustive.  
The way in which the platform \emph{presents} products and services to be searched by the buyers, therefore, crucially affects the market dynamics and outcomes.  
In most platforms, the providers/sellers set their own prices --- third-party sellers on Amazon, for example, set up their own prices, and so do hosts on Airbnb.
In wielding its power to mediate the interface, the platform must take into consideration both the sellers' pricing strategies and the buyers' search policies.

Our starting point is a monopolistic competition model where symmetric but differentiated sellers post their prices visible to all; a buyer must incur an inspection cost to determine her value for any specific seller, and this cost is the same for each seller.\footnote{As we explain later, this is essentially the classical model by \citet{wolinsky86true}, except that in our setting the prices are visible prior to search.  We note that prices usually do not take much effort to see in most online platforms.}
We observe that such a market does not have a pure equilibrium, i.e., no prices are stable, because the sellers are incentivized to undercut each other to be searched first by the buyer.
In practice, price volatility caused by ``algorithmic pricing'' has been voiced by the media \citep{Taft14, brown2016amazon} and has been a concern of consumers.  


In this work, we analyze a particularly simple scheme of presentation, wherein \emph{one} seller is made prominent, with drastically reduced inspection cost, while all the other sellers are treated equally.
The platform's rule for choosing the prominent seller sets up a mechanism, in response to which the sellers strategically set their prices.
We show that this presentation scheme, coupled with appropriate mechanisms, can stabilize prices at pure equilibria.
We further analyze the range of prices achievable at equilibria, and derive implications on welfare and consumer surplus.
An interesting discovery, among others, is that an increased inspection cost often increases the consumers' surplus, because the higher search barrier can induce sellers to lower their prices in order to gain prominence.

Before detailing our contributions, we take a moment to introduce Amazon's so-called \emph{Buy Box}, a typical interface design that features one prominent seller.
The Buy Box is an important motivation for our work.
% ; in the rest of the paper we refer to the prominent seller as the one \emph{in the Buy Box}.

\paragraph{The Amazon Buy Box}

\begin{figure}
\includegraphics[width=0.48\textwidth]{figures/buy_box_demo-1.png}
\Description{placeholder}
\includegraphics[width=0.48\textwidth]{figures/buy_box_demo-2.png}
\caption{Illustration of Amazon's Buy Box. 
\newline \normalfont{\textit{Top}: The Buy Box is highlighted in \textcolor{red}{red}. To view other sellers not in the Buy Box, a buyer needs to scroll down and click on the link we highlight in \textcolor{green}{green}.
\newline
\textit{Bottom}: A view of sellers not in the Buy Box.}}
\label{fig:buy_box_demo}
\Description{This screenshots displays when a user searches a book on Amazon. For the landing page. In red is the Buy Box section, which includes options such as 'Add to Cart' and 'Buy Now' buttons. To view alternative purchasing options from other sellers, users need to scroll down to the section marked in green.}
\end{figure}

When a buyer reaches a page on Amazon for a particular product, a {\em Buy Box} is shown (red box in Figure~\ref{fig:buy_box_demo}). 
There are typically multiple sellers for the product, but the Buy Box shows only one seller, with that seller's price and the buttons to press (either ``Add to Cart" or ``Buy now with 1-click") if the buyer were ready to purchase from the Buy Box seller.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.96\linewidth]{figures/buy_box_demo-1.png}
%     \caption{Buy Box interface demonstration. }
%     \label{fig:buy_box_demo-1}
%     \Description{description placeholder}
% \end{figure}
Below the Buy Box (and not always readily visible to a typical buyer), is an additional link (the green box in  Figure~\ref{fig:buy_box_demo}) to the other sellers of the same product (bottom of Figure~\ref{fig:buy_box_demo}), with some information about the prices they offer.
% \begin{figure}
%     \centering
%     \includegraphics[width=0.96\linewidth]{figures/buy_box_demo-2.png}
%     \caption{Outside the Buy Box.}
%     \label{fig:buy_box_demo-2}
%     \Description{description placeholder}
% \end{figure}
% See Figures~\ref{fig:BuyBox}
% and~\ref{fig:NonBuyBox}.

By presenting the sellers in this way, Amazon de facto reduces the inspection cost for the Buy Box seller, increasing the chance of a sale to this seller.
For the other sellers of this same product, Amazon has, for all practical purposes, increased the search cost. 

For the same product, the sellers' offers differ in aspects such as shipping time, location of seller, return and refund policy, product description (especially for used items), and whether they are ``fulfilled by Amazon''.
For any particular seller, a buyer can be certain that her value should be in a certain interval, but must spend effort to determine her exact value, according to her preference.


Placement in the Buy Box has a large impact on the demand for a seller's product, and Amazon's \emph{Buy Box mechanism} for determining the Buy Box seller has drawn attention from both the industry \citep{Bible} and academic works \citep{chen-algorithmic_pricing-2016}.  
The precise mechanism Amazon uses is proprietary information, and is generally considered to depend on many factors, including the sellers' prices, their past performances, etc..
Pricing on Amazon has long been known to involve software that helps to update prices dynamically; at least part of the drive for the incessant price changes is to compete for the Buy Box.

Wild price fluctuation on Amazon has been well documented~\citep{Taft14,brown2016amazon, hackernoon}; \citet{chen-algorithmic_pricing-2016} showed by simulation and by empirical observation that ``sellers that use algorithmic strategies to maintain low prices relative to their competitors are likely to gain a large advantage in the struggle to win the Buy Box''.
With fluctuating prices, not only should the sellers be constantly ready to change their prices, but buyers have also the added burden of uncertainty and should be strategic with the timing of purchase. 

In this work we build a theoretical framework and study a simplified scenario where the Buy Box mechanism only reacts to the prices set by the sellers.
We show that a mechanism which rewards the Buy Box to the most competitive price is intrinsically unstable in that no pure equilibrium exists.
We propose mechanisms admitting pure equilibria, study the range of equilibria prices, and derive welfare and surplus implications.

\paragraph{Our Contributions.}
We start with a model we call \emph{plain presentation} (without a prominent seller). 
 This is a monopolistic competition, where $m$ sellers offer differentiated goods/services at prices set by themselves.  
For each seller~$i$, a buyer has value $v_i$ drawn i.i.d.\@ from a known distribution~$F$.
We normalize values so that $F$ is supported on $[V, V + 1]$ for some $V > 0$; for many results we assume $V \geq 2$, and $c < \Ex{v_i} - V$.
For scenarios such as online retail platforms, these assumptions seem realistic.  (See further discussion in Section~\ref{sec:prelim}.)
The buyer knows~$F$ and can see the prices, but must incur an inspection cost~$c$ to be certain of any particular~$v_i$.
The buyer performs a sequential search, with free recall, in order to maximize her expected utility.
The optimal search policy is given by \citet{weitzman1979optimal}'s renowned index-based policy, which we present in detail in Section~\ref{sec:prelim}.
One feature of sequential search is that, whenever the buyer has found a value high enough, the search stops.
Sellers that are inspected earlier therefore have an advantage.

In this plain presentation model, the buyer's optimal policy goes over the sellers in the order of decreasing prices, which gives the sellers incentives to undercut each other.
We formally show that this market admits no pure symmetric equilibrium.\footnote{\citet{AZ11} mention in passing that ``this framework, where a consumer's match utility is independently distributed across firms, apparently does not lead to a tractable solution for how firms choose prices''.  Our proof may be seen as a formalization of this observation.}
Interestingly, for a market with two sellers, when $V \geq 2$, we show that even asymmetric pure equilibrium does not exist. 
For this result (Theorem~\ref{theorem:no_BB_no_eq}), we use a technique from \citet{armstrongAER}, which allows a nontrivial derivation of the sellers'  respective probabilities of selling had they been at an equilibrium;  a contradiction ensues from this calculation.

  When \emph{prominence} is given to a seller, e.g.\@ in the form of a Buy Box, we assume for simplicity that this seller has no inspection cost, i.e., a buyer always knows her value for this seller before any search, whereas every other seller still incurs an inspection cost~$c$.
As many platforms claim to aim for the lowest, most competitive prices, it is tempting to use a mechanism to induce low prices, e.g.\@ by giving prominence to only the seller with the lowest price.
It is not difficult to see that such an approach gives even more incentive for the sellers to undercut each other, and non-existence of equilibrium from the plain presentation model persists.

We therefore explore mechanisms that admit pure equilibria.
The first mechanism we consider is a \emph{dictator} --- the platform stipulates a price~$t$, and prominence is awarded to only sellers that post price~$t$; if there are multiple such sellers, pick one uniformly at random.
The mechanism is somewhat unnatural, but we show that it has the advantage that it encompasses all equilibria, in the sense that, if any natural mechanism (Definition~\ref{def:standard}) admits a pure symmetric equilibrium, the dictator mechanism admits the same equilibrium (by stipulating that price).
In Section~\ref{sec:implementable}, we completely characterize the range of equilibria realizable in the dictator mechanism (and hence all possible symmetric equilibria in natural mechanisms).  
Our main finding is that the prices implementable at equilibrium always constitute an interval.
The higher the inspection cost~$c$, the more likely a pure equilibrium exists and, when it does, the lower end of the interval is smaller, that is, the lower the implementable lowest price at equilibrium.
For the case of two sellers, we show more crisply that, as $c$ increases, the set of implementable prices grows inclusion-wise.
These findings suggest that, if a platform uses prominence solely to drive down prices, it is effective to increase the inspection cost for non-prominent sellers.

Towards more practical mechanisms, we consider \emph{threshold mechanisms}, which stipulate a price~$t$ and award prominence to sellers that post prices below~$t$; again, if there are multiple such sellers, pick one uniformly at random.
The threshold~$t$ acts similarly to a reserve price in auctions, but  the mechanism does not discriminate among sellers setting prices below~$t$.
This non-discrimination removes sellers' incentives to undercut each other, and makes it possible for pure equilibria to sustain.
If the platform uses a threshold mechanism and aims to drive down prices, it may lower the threshold~$t$ (to the extent that equilibrium still exists), rather than directly encourage competition among the sellers.
We again characterize the range of prices implementable at equilibria in threshold mechanisms (Theorem~\ref{thm:threshold}).
It is perhaps not surprising that there are settings where the dictator mechanism implements a larger range of prices than the threshold mechanism (Proposition~\ref{prop:dict-threshold-gap});
what we find interesting is that, whenever the threshold mechanism admits an equilibrium, the lowest price it is capable of maintaining at equilibrium is the same as that of the dictator mechanism (Corollary~\ref{cor:threshold}).
This suggests that, if the platform aims to drive down prices, the more practical-looking threshold mechanism is just as powerful as the stringent dictator mechanism, as long as the inspection cost is calibrated to a level that allows equilibria to exist.

Finally, we discuss welfare and consumer surplus at equilibria under the prominence mechanisms.
Since the inspection cost is a ``burned'' effort, and prices paid by the buyer and received by the sellers cancel out, the social welfare decreases as $c$ increases (Theorem~\ref{thm:welfare}).
The case of consumer surplus is more complex and interesting.
As $c$ increases, the lowest possible price implementable at equilibrium by a prominence mechanism decreases, but it is also more costly for the consumer to search.
The two factors work in opposite directions for the consumer surplus.
For many value distributions we experiment with, the consumer surplus largely increases as $c$ increases, but it is not necessarily the case that the surplus attains its maximum when $c$ is as large as possible.
In Theorem~\ref{thm:surplus-nonmonotone}, we derive a sufficient condition on~$F$ under which the consumer surplus is maximized at an inspection cost not at its maximum, if the platform implements the lowest equilibrium price.
We see this result as a proof of concept, illustrating that the relationship between the consumer surplus and the inspection cost is a complicated one.
% showing that increased inspection cost may enhance consumer's surplus due to intensified sellers' competition, even though at first glance it costs buyers more effort to acquire information.

\subsection*{Related Works}
The two works most closely related to the current work are \citet{AVZ09} and \citet{AZ11}, as both explicitly considered monopolistic competitions with search frictions and with prominent sellers, but both have key differences from our work.
\citet{AVZ09} consider a market where the a seller's price is invisible to the buyer unless the seller is inspected.
Price changes therefore do not directly affect the buyer's search order, which allows pure equilibria to exist.
We observe that in most online platforms the buyer sees sellers' prices quite easily, and take this as our starting point.
\citet{AZ11} study markets with visible prices, but circumvent the nonexistence of equilibria by considering negatively correlated values, which are stylized in a Hotelling model.  
For online shopping, we consider such negative correlation less well motivated, and stick to the classical i.i.d.\@ setting.
Moreover, we emphasize the mechanism design aspect in assigning prominence, in addition to static equilibrium analysis.
For other works on markets with search friction, we refer the reader to \citet{armstrong17survey} for a beautiful survey.

A small but growing number of works explicitly model buyers' search behavior to study platform presentations.
\citet{Chu_MS2020_PositionRankingAuction}, e.g., consider the ranking of heterogeneous products for a buyer whose search order is determined by this ranking, and they consider a multiobjective optimization that includes surplus and sales revenue.
\citet{Golrezaei_2022_MS_product_ranking} propose a two-stage search policy motivated by empirical evidence, and study product ranking in response to such search. % in order to maximize welfare and purchase probability.
\citet{Branco_MS2012_Search4ProductInfo} propose a continuous inspection procedure for a buyer to evaluate a single seller, and study the seller's optimal pricing in response.
Interestingly, in this setting very different from ours, it is also observed that increased search cost can sometimes benefit the buyer in equilibrium, due to the lower price set by the seller.

% The way we normalize the support of~$F$ to $[V, V + 1]$ and a proof in Section~\ref{sec:plain} both follow \citet{armstrongAER}, although the problem they study is on consumers' private signaling, quite distant from our setting.

% Beyond theoretical studies of search and presentation mechanisms, recent legal and regulatory research has also examined Amazon's Buy Box. For example, 
Amazon's Buy Box has drawn attention from researchers from many angles and disciplines.
Noticeably, legal scholars have studied consequences of algorithmic pricing 
\citep{MacKayWeinstein_DynamicPricingAlgorithms, Cavallo_OnlineCompetitionPricing} and anti-trust concerns of the Buy Box mechanism  \citep{Raval_SelfPreferencingBuyBox, DeMelis_AmazonAntitrustBuyBox}.
Our work takes the perspective of theory in market design, and stands at a distance from these.

% explore how algorithmic pricing affects competition and price adjustments across platforms like Amazon;  study Amazon’s Buy Box mechanism, with a focus on self-preferencing practices and potential antitrust concerns. 
% These works address broader regulatory challenges but provide complementary insights into platform strategies that impact both sellers and consumers.

\subsection*{Organization}
%The rest of the paper is organized as follows. 
In Section \ref{sec:prelim}, we present the monopolistic competition with search frictions, with a description of the buyer's optimal search procedure.
Section \ref{sec:plain} formally proves that the plain presentation sees no stable prices in equilibrium.
Section \ref{sec:buy-box} defines prominence mechanisms and presents the prices implementable at equilibria by the two mechanisms we study.
Section \ref{sec:welfare} analyzes welfare and consumer surplus under prominence mechanisms.
Most proofs are relegated to the appendix.


==> camera_ready/notation.tex <==
%% General machinery
\newcommand{\AutoAdjust}[3]{\mathchoice{ \left #1 #2  \right #3}{#1 #2 #3}{#1 #2 #3}{#1 #2 #3} }
\newcommand{\Xcomment}[1]{{}}
\newcommand{\eval}[1]{\left.#1\vphantom{\big|}\right|}
% \newcommand{\inteval}[1]{\Big[#1\Big]}
\newcommand{\InParentheses}[1]{\AutoAdjust{(}{#1}{)}}
\newcommand{\InBrackets}[1]{\AutoAdjust{[}{#1}{]}}% {\left[{#1}\right]}
\newcommand{\Ex}[2][]{\operatorname{\mathbf E}_{#1}\InBrackets{#2}}
\newcommand{\Prx}[2][]{\operatorname{\mathbf{Pr}}_{#1}\InBrackets{#2}}
\def\prob{\Prx}
\def\expect{\Ex}
\newcommand{\probq}[2]{x_{#1}\AutoAdjust{(}{#2}{)}}
\newcommand{\cumprobq}[2]{X_{#1}\AutoAdjust{(}{#2}{)}}
\newcommand{\super}[1]{^{(#1)}}
\newcommand{\dd}{\mathrm{d}}  % for integrals
\newcommand{\given}{\;\mid\;}
\newcommand{\eps}{\epsilon}
\newcommand{\OPT}{\mathrm{OPT}}
\newcommand{\EOPT}{\widetilde{\mathrm{OPT}}} % estimated OPT for discretization
\newcommand{\Dis}{D^S} % estimated OPT for discretization
\newcommand{\MAX}{\mathrm{MAX}}
\newcommand{\MAXV}{\textsc{MaxV}}
\newcommand{\MAXE}{\textsc{MaxE}}
\newcommand{\V}{\mathcal{V}}
% \newcommand{\R}{\mathcal{R}}
\newcommand{\DP}{\mathrm{DP}}
\newcommand{\A}{\mathcal{A}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\E}{\mathbf{E}}
\newcommand{\Sg}{\mathrm{Sg}}
% \newcommand{\T}{\mathcal{T}}
\newcommand{\DX}{v^S}
\newcommand{\Pandora}{PNOI } % a better name?
\newcommand{\TPandora}{T-PNOI } % a better name?
\newcommand{\TEPandora}{TE-PNOI }
\newcommand{\DPandora}{L-PNOI}
\newcommand{\Sdiscretized}{$S$-discretized}
\newcommand{\TState}{I_T}
\newcommand{\Ins}{B}
\newcommand{\DIns}{B^S}
\newcommand{\SH}{H_S}
\newcommand{\SG}{G_S}
\newcommand{\DV}{V^S}
\newcommand{\UP}{D^L}
\newcommand{\ActSet}{A}
\newcommand{\Tran}{\delta}
\newcommand{\TranP}{\Delta}
\newcommand{\RTran}{\gamma}
\newcommand{\Rank}{\mathrm{Rk}}
\newcommand{\Ch}{\mathrm{Ch}}
\newcommand{\fa}{\mathrm{Fa}}
\newcommand{\SUB}{Q}
\newcommand{\Round}{R}
\newcommand{\End}{\mathsf{end}}
\newcommand{\Tr}{\mathrm{Tr}}
\newcommand{\Indicator}[1]{\mathbf{1}\InBrackets{#1}}
\newcommand{\PI}{{W}}

% Very strange, it seems that \G is conflict with the EC22 style file. So I have to use \GG
\newcommand{\GG}{\mathcal{G}}

\newcommand{\poly}{\mathrm{poly}}
\newcommand{\maxp}{\Delta}
\newcommand{\Ut}{\mathrm{Utility}}
\newcommand{\Ls}{\mathrm{Loss}}
\newcommand{\Tbf}{T_{\textnormal{Bef}}}
\newcommand{\Tat}{T_{\textnormal{Aft}}}


% \newtheorem{thm}{Theorem}[section]
% \newtheorem{proposition}[thm]{Proposition}
% \newtheorem{lemma}[thm]{Lemma}
% \newtheorem{defn}[thm]{Definition}
% \newtheorem{claim}[thm]{Claim}
% \newtheorem{corollary}[thm]{Corollary}
% \newtheorem{definition}[thm]{Definition}
% \newtheorem{fact}[thm]{Fact}
% \newtheorem{remark}{Remark}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\supp}{supp}
\DeclareRobustCommand\iff{\;\Longleftrightarrow\;}

\newcommand{\noaccents}[1]{#1}
\newcommand{\newagentvar}[3][\noaccents]{%
\expandafter\newcommand\expandafter{\csname #2\endcsname}{#1{#3}}%
\expandafter\newcommand\expandafter{\csname #2s\endcsname}{#1{\boldsymbol{#3}}}%
\expandafter\newcommand\expandafter{\csname #2smi\endcsname}[1][i]{#1{\boldsymbol{#3}}_{-##1}}%
\expandafter\newcommand\expandafter{\csname #2i\endcsname}[1][i]{#1{#3}_{##1}}%
\expandafter\newcommand\expandafter{\csname #2ith\endcsname}[1][i]{#1{#3}_{(##1)}}%
}

\newcommand{\newvecagentvar}[3][\noaccents]{%
\expandafter\newcommand\expandafter{\csname #2\endcsname}{#1{\boldsymbol{#3}}}%
\expandafter\newcommand\expandafter{\csname #2s\endcsname}{#1{\boldsymbol{#3}}}%
\expandafter\newcommand\expandafter{\csname #2smi\endcsname}[1][i]{#1{\boldsymbol{#3}}_{-##1}}%
\expandafter\newcommand\expandafter{\csname #2i\endcsname}[1][i]{#1{\boldsymbol{#3}}_{##1}}%
\expandafter\newcommand\expandafter{\csname #2ith\endcsname}[1][i]{#1{#3}_{(##1)}}%
}

\newcommand{\authcom}[1]{\textcolor{magenta}{[#1]}}
\newcommand{\bluecom}[1]{\textcolor{blue}{[#1]}}

%% prelim

\newagentvar{alloc}{x}
\newagentvar{pay}{p}
\newagentvar{val}{v}
\newagentvar{util}{u}
\newagentvar{payment}{p}
\newagentvar{dist}{F}
\newcommand{\ps}{\mathbf{p}}

\newcommand{\gittins}{\tau}
\newcommand{\amorval}{\kappa}
\newcommand{\alg}{\mathcal{A}}
\newcommand{\truncalg}{\mathcal{B}}
\newcommand{\truncimpalg}{\mathcal{O}_{TE}}
\newcommand{\Dalg}{\mathcal{A}^S}
\newcommand{\threshold}{\theta}
\newcommand{\classnp}{\mathsf {NP}}
\newcommand{\classpspace}{\mathsf {PSPACE}}
\newcommand{\classp}{\mathsf {P}}
\newcommand{\leV}{\le_V}
\newcommand{\leW}{\le_W}

\newcommand{\image}{R}



==> conclusion.tex <==
We study the mechanism design problem for a two-sided online marketplace with search frictions on the buyer's side, exemplified by Amazon's business model and is canonical in digital economics. We propose a model that features multiple strategic sellers and utility maximizing buyers. Our model accounts for the buyer's optimal search behavior in the presence of inspection costs and sellers' strategic pricing behavior.
We characterize sellers' demand and revenue under these conditions, and analyze how the design of the Buy Box influences market outcomes, particularly focusing on price equilibria, social welfare, and consumer surplus.

The first part of our theoretical findings reveal that no symmetric equilibrium exists for markets with multiple sellers and that general equilibrium does not exist in the case of two sellers. This underscores the necessity of some mechanism to stabilize the market. 

Motivated by Amazon's approach, we study the design of Buy Box mechanisms. We first showed that the almost naive Lowest-Price-First mechanism does not sustain equilibrium. The inherent inspection cost boost Buy Box seller's demand, hence incentivizes sellers to constantly undercutting their prices to win the Buy Box. This finding aligns with the observed pricing chaos on Amazon, where frequent and significant price changes reflect the underlying instability in a market without an effective equilibrium mechanism.


To address this instability, we propose the Dictator-$t$ mechanism, which awards the Buy Box to sellers pricing at a pre-specified price point. This mechanism proves effective in being able to support the lowest equilibrium price among all anonymous mechanisms. We also examine the Threshold-$t$ mechanism, which selects sellers pricing below a specified threshold for the Buy Box. Although more flexible, this mechanism is less robust than the Dictator-$t$ mechanism, and does not achieve the same degree of low prices.

Furthermore, our analysis highlights the critical role of inspection costs in driving social welfare and consumer surplus. While in our model, higher inspection costs reduces social welfare, it lowers the incentive for buyers to conduct thorough searches, therefore, somewhat surprisingly, drives down equilibrium price and increases consumer surplus. This trade-off underscores the platform's strategic role in optimizing market outcomes by carefully calibrating the design of their display policy and user interface.

In conclusion, the Amazon Buy Box, when designed and implemented with consideration of inspection costs and appropriate mechanism, can significantly improve market efficiency and buyer utility. By establishing a model that incorporates both buyer and seller strategies, we provide a foundation for understanding how search frictions and platform design influence market outcomes. Future research can extend these insights by exploring dynamic pricing strategies and further empirical validation of the proposed mechanisms in diverse market settings. This study provides a critical framework for understanding the interplay between search frictions, platform design, and market outcomes in the digital economy.



